Improving LLM Group Fairness on Tabular Data via In-Context Learning

Large language models (LLMs) have been shown to be effective on tabular prediction tasks in the low-data regime, leveraging their internal knowledge and ability to learn from instructions and examples. However, LLMs can fail to generate predictions that satisfy group fairness, that is, produce equitable outcomes across groups. Critically, conventional debiasing approaches for natural language tasks do not directly translate to mitigating group unfairness in tabular settings. In this work, we systematically investigate four empirical approaches to improve group fairness of LLM predictions on tabular datasets, including fair prompt optimization, soft prompt tuning, strategic selection of few-shot examples, and self-refining predictions via chain-of-thought reasoning. Through experiments on four tabular datasets using both open-source and proprietary LLMs, we show the effectiveness of these methods in enhancing demographic parity while maintaining high overall performance. Our analysis provides actionable insights for practitioners in selecting the most suitable approach based on their specific requirements and constraints.

==> tables/prompt_details.tex <==
\begin{table*}[t!]
\centering
\begin{tabular}{|>{\raggedright\arraybackslash}p{5cm}|>{\raggedright\arraybackslash}p{10.5cm}|}
\hline
\textbf{Dataset} & \textbf{Prompt Template} \\
\hline
Adult \cite{becker1996adult} & You must follow the instructions to predict if income of an individual exceeds \$50K/yr. Generally, individuals who earn more than \$50K/yr tend to have higher levels of education (e.g., Bachelors or Prof-school), work in managerial or specialty occupations, and are married with a spouse. They also usually work longer hours per week and have higher capital gains. On the other hand, those earning less than or equal to \$50K/yr typically have lower levels of education (e.g., HS-grad), work in clerical or craft repair occupations, and may be single or married without a spouse. They also usually work fewer hours per week and have lower capital gains. 

You must provide an explanation and include answer enclosed in square brackets at the beginning of your response.
You must predict if the individual's income exceeds \$50K/yr. Answer with one of the following: [less than or equal to 50K] or [greater than 50K]. \\
\hline
German credit \cite{hofmann1994german} & age, gender, job, housing, savings status, checking status, credit amount, duration, and purpose \\
\hline
 ACS Income \cite{ding2021folktables} & gender, race, educational attainment, relationship, age, usual hours worked per week past 12 months, marital status, place of birth, class of worker, occupation
 \\
 \hline
 ACS Coverage \cite{ding2021folktables}& sex, race, educational attainment, military service, disability recode, total person's income, marital status, employment status recode, employment status of parents, gave birth to child within the past 12 months
 \\
\hline
\end{tabular}
\caption{Summary of datasets and features}
\label{tab:datasets}
\end{table*}

